Coping with Mistreatment in Fair Algorithms

Machine learning actively impacts our everyday life in almost all endeavors and domains such as healthcare, finance, and energy. As our dependence on the machine learning increases, it is inevitable that these algorithms will be used to make decisions that will have a direct impact on the society spanning all resolutions from personal choices to world-wide policies. Hence, it is crucial to ensure that (un)intentional bias does not affect the machine learning algorithms especially when they are required to take decisions that may have unintended consequences. Algorithmic fairness techniques have found traction in the machine learning community and many methods and metrics have been proposed to ensure and evaluate fairness in algorithms and data collection. In this paper, we study the algorithmic fairness in a supervised learning setting and examine the effect of optimizing a classifier for the Equal Opportunity metric. We demonstrate that such a classifier has an increased false positive rate across sensitive groups and propose a conceptually simple method to mitigate this bias. We rigorously analyze the proposed method and evaluate it on several real world datasets demonstrating its efficacy.

==> preface.tex <==
% This section allows us to modify preloaded package properties
\makeatletter
% These magic runes make comment's appear inline
% These also need to be above the other magic runes
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\usepackage{regexpatch}
\xpatchcmd{\@todo}{\setkeys{todonotes}{#1}}{\setkeys{todonotes}{inline,#1}}{}{}

% These magic runes make the new changes package work with comments
\usepackage{comment}
\let\wfs@comment@comment\comment
\let\comment\@undefined
\usepackage{changes}
\let\wfs@changes@comment\comment
\let\comment\@undefined
\newcommand\comment{%
    \ifthenelse{\equal{\@currenvir}{comment}}
    {\wfs@comment@comment}
    {\wfs@changes@comment}%
}
\makeatother

% Typical preloader time
\usepackage{arxiv}
\usepackage{hyperref}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{outlines}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{float}
\usepackage{nicefrac}
\usepackage{url}
\usepackage{booktabs}
\usepackage{listings}
\usepackage{todonotes}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{subfigure}
\lstset{
  basicstyle=\ttfamily,
  columns=fullflexible,
  frame=single,
  breaklines=true,
  tabsize=2,
  breakautoindent=true,
}
% nt -> env, disp text, [counter reset follow]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}{Proposition}[section]
% Changes Authors
\definechangesauthor[name="Ankit Kulshrestha", color=blue]{ak}
% \definechangesauthor[name="Ilya Tyagin", color=cyan]{it}
% \definechangesauthor[name="Justin Sybrandt", color=green]{js}
\definechangesauthor[name="Ilya Safro", color=red]{is}


\newcommand{\pymoliererepo}{
% \href{http://sybrandt.com/2020/agatha}
% {sybrandt.com/2020/agatha}
}
\newcommand{\pymoliere}{AGATHA}

% These are shortcuts for leaving specific changes comments
\newcommand{\note}[2]{\added[id=#1, comment={#2}]{}}

% Ankit's add, delete, replace
\newcommand{\Aak}[1]{\added[id=ak]{#1}}
\newcommand{\Dak}[1]{\deleted[id=ak]{#1}}
\newcommand{\Rak}[2]{\replaced[id=ak]{#1}{#2}}

% Justin's add, delete, replace
\newcommand{\Ajs}[1]{\added[id=js]{#1}}
\newcommand{\Djs}[1]{\deleted[id=js]{#1}}
\newcommand{\Rjs}[2]{\replaced[id=js]{#1}{#2}}

% ITyagin's add, delete replace
\newcommand{\Ait}[1]{\added[id=it]{#1}}
\newcommand{\Dit}[1]{\deleted[id=it]{#1}}
\newcommand{\Rit}[2]{\replaced[id=it]{#1}{#2}}

% ISafro's add, delete, replace
\newcommand{\Ais}[1]{\added[id=is]{#1}}
\newcommand{\Dis}[1]{\deleted[id=is]{#1}}
\newcommand{\Ris}[2]{\replaced[id=is]{#1}{#2}}

% THIS ALLOWS FOR CONDITIONAL COMMENTS
% \newif\ifthesis
% Comment/ un-comment as needed
% \thesisfalse
%\thesistrue

% Comment out a block of text for KDD (but keep for thesis) with this syntax:
% \ifthesis
% <Text to comment out>
% \else [Optional]
% <Optional replacement for KDD Version>
% \fi

\hyphenation{
    AG-A-THA
}

% These magic runes make everything denser
\setlength{\textfloatsep}{3pt}
\setlength{\floatsep}{3pt}
\setlength{\belowdisplayskip}{3pt} \setlength{\belowdisplayshortskip}{3pt}
\setlength{\abovedisplayskip}{3pt} \setlength{\abovedisplayshortskip}{3pt}

% \settopmatter{authorsperrow=4}

% \newcommand{\sysnameo}{AGATHA-O }
% \newcommand{\sysnamec}{AGATHA-C }
% \newcommand{\sysnamegp}{AGATHA-GP }
